Kernel-based Inference of Functions over Graphs

The study of networks has witnessed an explosive growth over the past decades with several ground-breaking methods introduced. A particularly interesting -- and prevalent in several fields of study -- problem is that of inferring a function defined over the nodes of a network. This work presents a versatile kernel-based framework for tackling this inference problem that naturally subsumes and generalizes the reconstruction approaches put forth recently by the signal processing on graphs community. Both the static and the dynamic settings are considered along with effective modeling approaches for addressing real-world problems. The herein analytical discussion is complemented by a set of numerical examples, which showcase the effectiveness of the presented techniques, as well as their merits related to state-of-the-art methods.

==> include.tex <==

% Also note that the "draftcls" or "draftclsnofoot", not "draft", option
% should be used if it is desired that the figures are to be displayed in
% draft mode.
%



% *** MISC UTILITY PACKAGES ***
%
%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%   % dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/tex-archive/macros/latex/contrib/oberdiek/
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.






% *** CITATION PACKAGES ***
%
\usepackage{cite}
% cite.sty was written by Donald Arseneau
% V1.6 and later of IEEEtran pre-defines the format of the cite.sty package
% \cite{} output to follow that of IEEE. Loading the cite package will
% result in citation numbers being automatically sorted and properly
% "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% \cite will automatically add leading space, if needed. Use cite.sty's
% noadjust option (cite.sty V3.8 and later) if you want to turn this off.
% cite.sty is already installed on most LaTeX systems. Be sure and use
% version 4.0 (2003-05-27) and later if using hyperref.sty. cite.sty does
% not currently provide for hyperlinked citations.
% The latest version can be obtained at:
% http://www.ctan.org/tex-archive/macros/latex/contrib/cite/
% The documentation is contained in the cite.sty file itself.






% *** GRAPHICS RELATED PACKAGES ***
%
%% \ifCLASSINFOpdf
%%   % \usepackage[pdftex]{graphicx}
%%   % declare the path(s) where your graphic files are
%%   % \graphicspath{{../pdf/}{../jpeg/}}
%%   % and their extensions so you won't have to specify these with
%%   % every instance of \includegraphics
%%   % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
%% \else
%%   % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
%%   % will default to the driver specified in the system graphics.cfg if no
%%   % driver is specified.
%%   % \usepackage[dvips]{graphicx}
%%   % declare the path(s) where your graphic files are
%%   % \graphicspath{{../eps/}}
%%   % and their extensions so you won't have to specify these with
%%   % every instance of \includegraphics
%%   % \DeclareGraphicsExtensions{.eps}
%% \fi

% graphicx was written by David Carlisle and Sebastian Rahtz. It is
% required if you want graphics, photos, etc. graphicx.sty is already
% installed on most LaTeX systems. The latest version and documentation can
% be obtained at: 
% http://www.ctan.org/tex-archive/macros/latex/required/graphics/
% Another good source of documentation is "Using Imported Graphics in
% LaTeX2e" by Keith Reckdahl which can be found as epslatex.ps or
% epslatex.pdf at: http://www.ctan.org/tex-archive/info/
%
% latex, and pdflatex in dvi mode, support graphics in encapsulated
% postscript (.eps) format. pdflatex in pdf mode supports graphics
% in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% not a bitmapped formats (.jpeg, .png). IEEE frowns on bitmapped formats
% which can result in "jaggedy"/blurry rendering of lines and letters as
% well as large increases in file sizes.
%
% You can find documentation about the pdfTeX application at:
% http://www.tug.org/applications/pdftex





% *** MATH PACKAGES ***
%
%\usepackage[cmex10]{amsmath}
% A popular package from the American Mathematical Society that provides
% many useful and powerful commands for dealing with mathematics. If using
% it, be sure to load this package with the cmex10 option to ensure that
% only type 1 fonts will utilized at all point sizes. Without this option,
% it is possible that some math symbols, particularly those within
% footnotes, will be rendered in bitmap form which will result in a
% document that can not be IEEE Xplore compliant!
%
% Also, note that the amsmath package sets \interdisplaylinepenalty to 10000
% thus preventing page breaks from occurring within multiline equations. Use:
%\interdisplaylinepenalty=2500
% after loading amsmath to restore such page breaks as IEEEtran.cls normally
% does. amsmath.sty is already installed on most LaTeX systems. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/tex-archive/macros/latex/required/amslatex/math/





% *** SPECIALIZED LIST PACKAGES ***
%
%\usepackage{algorithmic}
% algorithmic.sty was written by Peter Williams and Rogerio Brito.
% This package provides an algorithmic environment fo describing algorithms.
% You can use the algorithmic environment in-text or within a figure
% environment to provide for a floating algorithm. Do NOT use the algorithm
% floating environment provided by algorithm.sty (by the same authors) or
% algorithm2e.sty (by Christophe Fiorio) as IEEE does not use dedicated
% algorithm float types and packages that provide these will not provide
% correct IEEE style captions. The latest version and documentation of
% algorithmic.sty can be obtained at:
% http://www.ctan.org/tex-archive/macros/latex/contrib/algorithms/
% There is also a support site at:
% http://algorithms.berlios.de/index.html
% Also of interest may be the (relatively newer and more customizable)
% algorithmicx.sty package by Szasz Janos:
% http://www.ctan.org/tex-archive/macros/latex/contrib/algorithmicx/




% *** ALIGNMENT PACKAGES ***
%
%\usepackage{array}
% Frank Mittelbach's and David Carlisle's array.sty patches and improves
% the standard LaTeX2e array and tabular environments to provide better
% appearance and additional user controls. As the default LaTeX2e table
% generation code is lacking to the point of almost being broken with
% respect to the quality of the end results, all users are strongly
% advised to use an enhanced (at the very least that provided by array.sty)
% set of table tools. array.sty is already installed on most systems. The
% latest version and documentation can be obtained at:
% http://www.ctan.org/tex-archive/macros/latex/required/tools/


%\usepackage{mdwmath}
%\usepackage{mdwtab}
% Also highly recommended is Mark Wooding's extremely powerful MDW tools,
% especially mdwmath.sty and mdwtab.sty which are used to format equations
% and tables, respectively. The MDWtools set is already installed on most
% LaTeX systems. The lastest version and documentation is available at:
% http://www.ctan.org/tex-archive/macros/latex/contrib/mdwtools/


% IEEEtran contains the IEEEeqnarray family of commands that can be used to
% generate multiline equations as well as matrices, tables, etc., of high
% quality.


%\usepackage{eqparbox}
% Also of notable interest is Scott Pakin's eqparbox package for creating
% (automatically sized) equal width boxes - aka "natural width parboxes".
% Available at:
% http://www.ctan.org/tex-archive/macros/latex/contrib/eqparbox/





% *** SUBFIGURE PACKAGES ***
%\usepackage[tight,footnotesize]{subfigure}
% subfigure.sty was written by Steven Douglas Cochran. This package makes it
% easy to put subfigures in your figures. e.g., "Figure 1a and 1b". For IEEE
% work, it is a good idea to load it with the tight package option to reduce
% the amount of white space around the subfigures. subfigure.sty is already
% installed on most LaTeX systems. The latest version and documentation can
% be obtained at:
% http://www.ctan.org/tex-archive/obsolete/macros/latex/contrib/subfigure/
% subfigure.sty has been superceeded by subfig.sty.



%\usepackage[caption=false]{caption}
%\usepackage[font=footnotesize]{subfig}
% subfig.sty, also written by Steven Douglas Cochran, is the modern
% replacement for subfigure.sty. However, subfig.sty requires and
% automatically loads Axel Sommerfeldt's caption.sty which will override
% IEEEtran.cls handling of captions and this will result in nonIEEE style
% figure/table captions. To prevent this problem, be sure and preload
% caption.sty with its "caption=false" package option. This is will preserve
% IEEEtran.cls handing of captions. Version 1.3 (2005/06/28) and later 
% (recommended due to many improvements over 1.2) of subfig.sty supports
% the caption=false option directly:
%\usepackage[caption=false,font=footnotesize]{subfig}
%
% The latest version and documentation can be obtained at:
% http://www.ctan.org/tex-archive/macros/latex/contrib/subfig/
% The latest version and documentation of caption.sty can be obtained at:
% http://www.ctan.org/tex-archive/macros/latex/contrib/caption/




% *** FLOAT PACKAGES ***
%
\usepackage{fixltx2e}
% fixltx2e, the successor to the earlier fix2col.sty, was written by
% Frank Mittelbach and David Carlisle. This package corrects a few problems
% in the LaTeX2e kernel, the most notable of which is that in current
% LaTeX2e releases, the ordering of single and double column floats is not
% guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
% single column figure to be placed prior to an earlier double column
% figure. The latest version and documentation can be found at:
% http://www.ctan.org/tex-archive/macros/latex/base/



%\usepackage{stfloats}
% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% the ability to do double column floats at the bottom of the page as well
% as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% LaTeX2e). It also provides a command:
%\fnbelowfloat
% to enable the placement of footnotes below bottom floats (the standard
% LaTeX2e kernel puts them above bottom floats). This is an invasive package
% which rewrites many portions of the LaTeX2e float routines. It may not work
% with other packages that modify the LaTeX2e float routines. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/tex-archive/macros/latex/contrib/sttools/
% Documentation is contained in the stfloats.sty comments as well as in the
% presfull.pdf file. Do not use the stfloats baselinefloat ability as IEEE
% does not allow \baselineskip to stretch. Authors submitting work to the
% IEEE should note that IEEE rarely uses double column equations and
% that authors should try to avoid such use. Do not be tempted to use the
% cuted.sty or midfloat.sty packages (also by Sigitas Tolusis) as IEEE does
% not format its papers in such ways.


%\ifCLASSOPTIONcaptionsoff
%  \usepackage[nomarkers]{endfloat}
% \let\MYoriglatexcaption\caption
% \renewcommand{\caption}[2][\relax]{\MYoriglatexcaption[#2]{#2}}
%\fi
% endfloat.sty was written by James Darrell McCauley and Jeff Goldberg.
% This package may be useful when used in conjunction with IEEEtran.cls'
% captionsoff option. Some IEEE journals/societies require that submissions
% have lists of figures/tables at the end of the paper and that
% figures/tables without any captions are placed on a page by themselves at
% the end of the document. If needed, the draftcls IEEEtran class option or
% \CLASSINPUTbaselinestretch interface can be used to increase the line
% spacing as well. Be sure and use the nomarkers option of endfloat to
% prevent endfloat from "marking" where the figures would have been placed
% in the text. The two hack lines of code above are a slight modification of
% that suggested by in the endfloat docs (section 8.3.1) to ensure that
% the full captions always appear in the list of figures/tables - even if
% the user used the short optional argument of \caption[]{}.
% IEEE papers do not typically make use of \caption[]'s optional argument,
% so this should not be an issue. A similar trick can be used to disable
% captions of packages such as subfig.sty that lack options to turn off
% the subcaptions:
% For subfig.sty:
% \let\MYorigsubfloat\subfloat
% \renewcommand{\subfloat}[2][\relax]{\MYorigsubfloat[]{#2}}
% For subfigure.sty:
% \let\MYorigsubfigure\subfigure
% \renewcommand{\subfigure}[2][\relax]{\MYorigsubfigure[]{#2}}
% However, the above trick will not work if both optional arguments of
% the \subfloat/subfig command are used. Furthermore, there needs to be a
% description of each subfigure *somewhere* and endfloat does not add
% subfigure captions to its list of figures. Thus, the best approach is to
% avoid the use of subfigure captions (many IEEE journals avoid them anyway)
% and instead reference/explain all the subfigures within the main caption.
% The latest version of endfloat.sty and its documentation can obtained at:
% http://www.ctan.org/tex-archive/macros/latex/contrib/endfloat/
%
% The IEEEtran \ifCLASSOPTIONcaptionsoff conditional can also be used
% later in the document, say, to conditionally put the References on a 
% page by themselves.





% *** PDF, URL AND HYPERLINK PACKAGES ***
%
%\usepackage{url}
% url.sty was written by Donald Arseneau. It provides better support for
% handling and breaking URLs. url.sty is already installed on most LaTeX
% systems. The latest version can be obtained at:
% http://www.ctan.org/tex-archive/macros/latex/contrib/misc/
% Read the url.sty source comments for usage information. Basically,
% \url{my_url_here}.





% *** Do not adjust lengths that control margins, column widths, etc. ***
% *** Do not use packages that alter fonts (such as pslatex).         ***
% There should be no need to do such things with IEEEtran.cls V1.6 and later.
% (Unless specifically asked to do so by the journal or conference you plan
% to submit to, of course. )



% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation Results}
%\label{fig_sim}
%\end{figure}

% Note that IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command, the
% \label for the overall figure must come after \caption.
% \hfil must be used as a separator to get equal spacing.
% The subfigure.sty package works much the same way, except \subfigure is
% used instead of \subfloat.
%
%\begin{figure*}[!t]
%\centerline{\subfloat[Case I]\includegraphics[width=2.5in]{subfigcase1}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{subfigcase2}%
%\label{fig_second_case}}}
%\caption{Simulation results}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.


% An example of a floating table. Note that, for IEEE style tables, the 
% \caption command should come BEFORE the table. Table text will default to
% \footnotesize as IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that IEEE does not put floats in the very first column - or typically
% anywhere on the first page for that matter. Also, in-text middle ("here")
% positioning is not used. Most IEEE journals use top floats exclusively.
% Note that, LaTeX2e, unlike IEEE journals, places footnotes above bottom
% floats. This can be corrected via the \fnbelowfloat command of the
% stfloats package.


% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://www.ctan.org/tex-archive/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)




%% biography section
%% % 
%% % If you have an EPS/PDF photo (graphicx package needed) extra braces are
%% % needed around the contents of the optional argument to biography to prevent
%% % the LaTeX parser from getting confused when it sees the complicated
%% % \includegraphics command within an optional argument. (You could create
%% % your own custom macro containing the \includegraphics command to make things
%% % simpler here.)
%% %\begin{biography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
%% % or if you just want to reserve a space for a photo:

%% \begin{IEEEbiography}{Michael Shell}
%% Biography text here.
%% \end{IEEEbiography}

%% % if you will not have a photo at all:
%% \begin{IEEEbiographynophoto}{John Doe}
%% Biography text here.
%% \end{IEEEbiographynophoto}

%% % insert where needed to balance the two columns on the last page with
%% % biographies
%% %\newpage

%% \begin{IEEEbiographynophoto}{Jane Doe}
%% Biography text here.
%% \end{IEEEbiographynophoto}

%% % You can push biographies down or up by placing
%% % a \vfill before or after them. The appropriate
%% % use of \vfill depends on what kind of text is
%% % on the last page and whether or not the columns
%% % are being equalized.

%% %\vfill

%% % Can be used to pull up biographies so that the bottom of the last one
%% % is flush with the other column.
%% %\enlargethispage{-5in}



\usepackage{graphicx}

%\usepackage{subfig}  % I have read that subcaption works better than subfig
%\usepackage{subcaption}              %subfigures with \mbox and \subfigure[]

\usepackage[utf8]{inputenc}


%\usepackage[spanish]{babel}
%\usepackage[galician]{babel}

\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{mathtools}
%\usepackage{amsthm}   % use \qedhere to place the QED 
                      % symbol at the end of a math line
                      % or environment {proof}.

\usepackage{amssymb}

\usepackage{bm}
%\usepackage{cancel} % use \cancel{expression}, \xcancel{}, etc

\usepackage{color,verbatim}
\usepackage{multirow}
\usepackage{accents}

\usepackage{theoremref}
% use \thlabel{} and \thref{}


%\usepackage{balance}  % if you want to balance the height of the two columns
% at the last page write \balance on the first column of the last page.

\usepackage{flushend}

\usepackage{url}

%\usepackage{lineno} %-> you should copy the .sty files to the current
% folder and include \linenumbers after \begin{document}. Note, the
% package does not work well with environment *equation*. It is better
% to use the environment *eqnarray* for equations.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CUSTOMIZATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\def\figurename{Figura}
%\def\refname{Referencias}


%% \topmargin 0truein
%% \topskip 0truein
%% \headheight 0truein
%% \headsep 0.5truein
%% %\footheight 0truein
%% \oddsidemargin 0.0in
%% \evensidemargin 0.0in
%% \textwidth 6.5in
%% \textheight 8.5in

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ENVIRONMENTS%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newenvironment{mycolorexample}
        { \begin{colbox}{orange}
\textit{Example:}\\ \small    }
        {   \end{colbox}  }

\newenvironment{myexample}
        {\textit{Example:}\\ \small    }
        {     }

\newenvironment{mycolorinformalproof}
        {% \begin{colbox}{gray}
 \small\color{darkblue}    \textit{Informal Proof:}\\}
        { % \end{colbox}  
}

\newenvironment{mycolorproof}
        {% \begin{colbox}{gray}
 \small\color{darkblue}    \textit{Proof:}\\}
        { % \end{colbox}  
}


\newenvironment{mycolortheorem}
        { \begin{colbox}{lightred}
\color{black}    \begin{mytheorem}}
        {\end{mytheorem}
 \end{colbox}  
}

\newenvironment{mycolorlemma}
        { \begin{colbox}{lightgray}
\color{black}    \begin{mylemma}}
        {\end{mylemma}
 \end{colbox}  
}



\newenvironment{mycolordefinition}
        { \begin{colbox}{lightgreen}
\color{black}    \begin{mydefinition}}
        {\end{mydefinition}
 \end{colbox}  
}


\newenvironment{mycolorproposition}
        { \begin{colbox}{lightgray}
\color{black}    \begin{myproposition}}
        {\end{myproposition}
 \end{colbox}  
}

\newenvironment{mycolorcorollary}
        { \begin{colbox}{lightgray}
\color{black}    \begin{mycorollary}}
        {\end{mycorollary}
 \end{colbox}  
}




\newenvironment{mycolormnemonic}
        { \begin{colbox}{lightblue}
\color{black}    \textbf{Mnemonic:}}
        {
 \end{colbox}  
}



\newenvironment{mycolorremark}
        { \begin{colbox}{lightgray}
\color{black}    \begin{myremark}}
        {\end{myremark}
 \end{colbox}  
}



\newenvironment{mycolorproblemstatement}
        { \begin{colbox}{purple}
\color{black}    \begin{myproblemstatement}}
        {\end{myproblemstatement}
 \end{colbox}  
}



\newcommand{\mycolorbox}[2]{
 \begin{colbox}{purple}
\color{black}    
\textbf{#1}\\
#2
 \end{colbox}  
}





\newcounter{rulecounter}
\newcommand{\resetrule}{ \setcounter{rulecounter}{0}}
\resetrule
\newenvironment{ruleenv}[1]
               {\refstepcounter{rulecounter}
               \par\noindent \textbf{Rule \arabic{rulecounter}:} \textit{#1}\\}
               {  }





\newenvironment{algoritm}[1]
               {\vspace{0.3in}
                 \begin{center}
                   \parbox{6in}{#1}
                 \end{center}
                 \vspace{0.15in}
                 \hrule
                 \begin{enumerate}}
               {
                 \end{enumerate}
                 \hrule
                 \vspace{0.3in}}

\newenvironment{exercise}[1]
               {\par\noindent\underline{\textbf{Exercise #1}}\bf\par\noindent}
               {}

\newenvironment{question}
               {\par\noindent \begin{itshape}\par\noindent\begin{itemize}\item \bf}
               {\end{itemize}\end{itshape}}

\newenvironment{mysolution}
               {\par\noindent\underline{{Solution}}\par\indent}
               {\begin{flushright} $\Box$ \end{flushright}}


% Color box 
\newsavebox{\selvestebox}
\newenvironment{colbox}[1]
  {\newcommand\colboxcolor{#1}%
   \begin{lrbox}{\selvestebox}%
   \begin{minipage}{\dimexpr\columnwidth-2\fboxsep\relax}}
  {\end{minipage}\end{lrbox}%
   \begin{center}
   \colorbox{\colboxcolor}{\usebox{\selvestebox}}
   \end{center}}

% Colors
\definecolor{orange}{rgb}{1,0.8,0}
\definecolor{gray}{rgb}{.9,0.9,0.9}
\definecolor{darkgray}{rgb}{.3,0.3,0.3}
\definecolor{darkblue}{rgb}{.1,0.0,0.3}
\definecolor{lightblue}{rgb}{0.7,0.7,1}
\definecolor{lightred}{rgb}{1,0.7,.7}
\definecolor{purple}{RGB}{204,153,255}
\definecolor{lightgray}{rgb}{.95,0.95,0.95}
\definecolor{lightgreen}{rgb}{0.3,0.5,0.3}
\definecolor{darkgreen}{rgb}{0.05,0.3,0.05}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% text mode
\newcommand{\vs}{\emph{vs.}}
\newcommand{\ea}{\emph{et al.}}
\newcommand{\ra}{$\rightarrow$~}
\newcommand{\Ra}{$\Rightarrow$~}

% math mode
\newcommand{\fourierpair}{~\xleftrightarrow{~\mathcal{F}~}~}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\ubbm}[1]{\ubar{\bm{#1}}}
\newcommand{\brackets}[1]{\left\{#1\right\}}
%\newcommand{\q}[1]{\mbox{$q^{- #1}$}}
\newcommand{\bbm}[1]{{\bar{\bm #1}}}
\newcommand{\dbbm}[1]{{\dbar{\bm #1}}}
\newcommand{\dbar}[1]{{\bar{\bar{ #1}}}}
\newcommand{\tbm}[1]{{\tilde{\bm #1}}}
\newcommand{\cbm}[1]{{\check{\bm #1}}}
\newcommand{\hbm}[1]{{\hat{\bm #1}}}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\msqrt}{^{1/2}}
\newcommand{\msqrtinv}{^{-1/2}}

\newcommand{\ffield}{\mathbb{F}}
\newcommand{\cfield}{\mathbb{C}}
\newcommand{\rfield}{\mathbb{R}}
\newcommand{\vect}{\mathop{\rm vec}}
\newcommand{\vectinv}{\mathop{\rm vec}^{-1}}
\newcommand{\re}[1]{\mathop{\rm Re}\brackets{#1}}
\newcommand{\im}[1]{\mathop{\rm Im}\brackets{#1}}
\newcommand{\cov}[2]{\mathop{\rm Cov}\left\{#1,#2\right\}}
\newcommand{\diag}[1]{\mathop{\rm diag}\brackets{#1}}
\newcommand{\toep}[1]{\mathop{\rm toep}\brackets{#1}}
\newcommand{\bdiag}[1]{\mathop{\rm bdiag}\brackets{#1}}
\newcommand{\diagnb}{\mathop{\rm diag}}
\newcommand{\vectnb}{\mathop{\rm vec}}
\newcommand{\rankb}[1]{\mathop{\rm rank}\brackets{#1}}
\newcommand{\ranknb}{\mathop{\rm rank}}
\newcommand{\rank}{\mathop{\rm rank}}
\newcommand{\krank}{\mathop{\rm krank}}
\newcommand{\lambdamax}{\lambda_\text{max}}
\newcommand{\lambdamin}{\lambda_\text{mmin}}
\newcommand{\dimf}{\mathop{\rm dim}_\ffield}
\newcommand{\dimr}{\mathop{\rm dim}_\rfield}
\newcommand{\dimc}{\mathop{\rm dim}_\cfield}
\newcommand{\spanv}{\mathop{\rm span}}
\newcommand{\spanvf}{\spanv_{\ffield}}
\newcommand{\spanvr}{\spanv_{\rfield}}
\newcommand{\spanvc}{\spanv_{\cfield}}
\newcommand{\vecv}{\mathop{\rm vec}}
\newcommand{\defect}[1]{\mathop{\rm def}\brackets{#1}}
\newcommand{\range}[1]{\mathcal{R}\brackets{#1}}
\newcommand{\nullspace}[1]{\mathcal{N}\brackets{#1}}
%\newcommand{\snr}{\mathop{\rm SNR}}
\newcommand{\tr}[1]{\mathop{\rm Tr}\left(#1\right)}
\newcommand{\trnb}{\mathop{\rm Tr}}
%\newcommand{\etr}[1]{\mathop{\mathrm{Etr}}\left\{#1\right\}}
\newcommand{\etr}[1]{\operatorname{etr}\left\{#1\right\}}
\newcommand{\etrnb}{\operatorname{etr}}
\newcommand{\trs}[1]{\mathop{\rm Tr^2}\left(#1\right)}
\newcommand{\sign}[1]{\mathop{\rm sign}\brackets{#1}}
\newcommand{\GM}{\mathop{\rm GM}}
\newcommand{\rect}{\mathop{\rm rect}}
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\newcommand{\sinc}{\mathop{\rm sinc}}

%% \newcommand{\define}{
%%   \begin{array}{c}
%%     \text{\tiny{$\Delta$}} \\[-0.3cm]
%%     = \\[-0.3cm]
%%     ~
%%   \end{array}
%% }
 \newcommand{\define}{\triangleq}
% \newcommand{\conv}{\star} % convolution
\newcommand{\conv}{{\hspace{3pt}\star}\hspace{3pt}} % convolution

\newcommand{\equalls}{
  \begin{array}{c}
    \text{\tiny{\text{LS}}} \\[-0.5cm]
    = \\[-0.3cm]
    ~
  \end{array}
}

\newcommand{\intinfty}{\int_{-\infty}^\infty}

\newcommand{\zmo}{z^{-1}}
\newcommand{\ellon}{$\ell^1$-norm}
\newcommand{\elltn}{$\ell^2$-norm}

\newcommand{\prob}[1]{\mathop{\textrm{P}} \brackets{#1} }
\newcommand{\probnb}{\mathop{\textrm{P}} }
\newcommand{\expected}[1]{\mathop{\textrm{E}}\brackets{#1} }
\newcommand{\expectednb}{\mathop{\textrm{E}}\nolimits}
\newcommand{\expectedwrt}[2]{\mathop{\textrm{E}}\nolimits_{#1}\{#2\}}
\newcommand{\expb}[1]{\exp \brackets{#1} }
\newcommand{\var}[1]{\mathop{\textrm{Var}}\brackets{#1} }

\newcommand{\pd}{P_\text{D}}
\newcommand{\pfa}{P_\text{FA}}
\newcommand{\hz}{{\mathcal{H}_0}}
\newcommand{\ho}{{\mathcal{H}_1}}
\newcommand{\hi}{{\mathcal{H}_i}}
\newcommand{\decide}{\mathop{\gtrless}^{\mathcal{H}_1}_{\mathcal{H}_0}}
\newcommand{\decideinv}{\mathop{\gtrless}^{\mathcal{H}_0}_{\mathcal{H}_1}}
\newcommand{\minimize}{\mathop{\text{minimize}}}
\newcommand{\maximize}{\mathop{\text{maximize}}}
\newcommand{\optimize}{\mathop{\text{optimize}}}
\newcommand{\st}{\mathop{\text{s.t.}}}
\newcommand{\subjectto}{\mathop{\text{s.t}}}
\newcommand{\image}{\mathop{\text{image}}}
\newcommand{\ejo}{(e^{j\omega})}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{myproposition}{Proposition}
\newtheorem{myremark}{Remark}
\newtheorem{myproblemstatement}{Problem Statement}
\newtheorem{mylemma}{Lemma}
\newtheorem{mytheorem}{Theorem}
\newtheorem{mydefinition}{Definition}
\newtheorem{mycorollary}{Corollary}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% TEMPLATES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
%% COUNTERS:
%%
%% \addtocounter{counter}{value} increments counter by 
%%     the amount, which can be negative
%% \alph{counter}, \Alph{counter} print the value of
%%      the counter as a lower or upper case letter.
%% \arabic{counter} print the value of the counter as an 
%%      arabic number \fnsymbol{counter} print the counter 
%%      as a footnote symbol 
%% \newcounter define a new counter 
%% \roman{counter}, \Roman{counter} print the value of the
%%     counter as a roman letter using lower or upper case
%%     letters 
%% \setcounter{counter}{value} assign the value to the
%%     counter 
%% \usecounter{counter} to be used in list environment.  
%% \value{counter} get the value of the counter.
%% \refstepcounter{counter} increments and makes label 
%%     command take its value


%%   Illustrate functions over sets
%%    
%%    \begin{align}
%%      \begin{array}{ccccc}
%%        V&\multicolumn{3}{c}{\xrightarrow{\hspace{2cm}f\hspace{2cm}}} &\mathbb{R}\\
%%        V&\xrightarrow{~f_1~}&W&\xrightarrow{~f_2~} &\mathbb{R}\\
%%        v&\rightarrow&w=f_1(v)&\rightarrow &f_2(w)
%%      \end{array}
%%    \end{align}



%% 
% you can use \xleftarrow{something} to display an 
% arrow with text above.
%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % % % % % % % % % % % % % % % % % % % % % % % % 
%\abstract{}

%\begin{exercise}{1: Exercise name}
%\end{exercise}

%\begin{question}
%\end{question}

%\begin{solution}
%\end{solution}

%\clearpage

%\displaystyle : in arrays of equations, placed before the expression,
%                it prevents it from becoming smaller.

%\begin{figure}[bhtp]
%  \centering
%  \includegraphics[width=1.0\textwidth]{route.png or route.jpg}
%  \caption{    }
%  \label{  }
%\end{figure}


%% \begin{figure}
%% \begin{minipage}[b]{.5\linewidth}
%% \centering\large A
%% \subcaption{A subfigure}\label{fig:1a}
%% \end{minipage}%
%% \begin{minipage}[b]{.5\linewidth}
%% \centering\large B
%% \subcaption{Another subfigure}\label{fig:1b}
%% \end{minipage}
%% \caption{A figure}\label{fig:1}
%% \end{figure}


%% \begin{figure}[bhtp]
%%  \centering
%%  \subfloat[one]{
%%    \label{}
%%    \includegraphics[width=1.0\textwidth]{route.png or route.jpg}
%%  } %\\ -> to arrange vertically
%%  \subfloat[two]{
%%    \label{}
%%    \includegraphics[width=1.0\textwidth]{route.png or route.jpg}
%%  } % etc
%%  \caption{    }
%%  \label{  }
%% \end{figure}


% to add a figure from xfig export it as *Combined PS/LaTeX (both
% parts)* (=> extension .pstex). Then substitute
% \includegraphics... in this file by \input{filename.pstex_t}


%   \begin{table}[bhtp] % table as image
%     \centering
%     \includegraphics[width=1.0\textwidth]{route.png etc}
%     \caption{    }
%     \label{ }
%   \end{table}

% To include multiline equations in tables use, inside a cell:
%% \begin{center}
%%    $\begin{aligned}
%%    exp1 & exp2 \\
%%    exp3 & exp4 \\
%%    \end{aligned}$
%% \end{center}

% aligned also allows to use \boxed{} for multi-line equations

%% z = \overbrace{
%%     \underbrace{x}_\text{real} +
%%     \underbrace{iy}_\text{imaginary}
%%    }^\text{complex number}

%%  \renewcommand{\refname}{} % to remove the word ``REFERENCES''
%%  from the bibliography.


%% This is to attach a letter to the reference numbers, e.g. [2],[33]  by [P2],[P33]
%% \makeatletter
%% \renewcommand*{\@biblabel}[1]{[P#1]}
%% \makeatother
%% \renewcommand\citeform[1]{P#1}




%% \usepackage{algorithmic}
%% \usepackage[ruled,vlined,resetcount]{algorithm2e}
%
%% \begin{algorithm}                   
%% \caption{Censored Algorithm}
%% \label{algo:1}    
%% \begin{minipage}{200cm}
%% \begin{algorithmic}[1]
%% \STATE Initialize 
%% \FOR{$n=1,2,\ldots$}
%% \IF{uuu}
%% \STATE Estimate
%% \ENDIF
%% \STATE Set 
%% \ENDFOR
%% \STATE Set 
%% \end{algorithmic}
%% \end{minipage}
%% \end{algorithm}



% \begin{center}
%   \begin{tabular}{|c | c | c|}
%     \hline
%      &  & \\
%     \hline
%     \hline
%      &  & \\
%     \hline
%     &  & \\
%     \hline
%     &  & \\
%     \hline
%   \end{tabular}
% \end{center}

%% use \renewcommand{\arraystretch}{2} before to make rows  higher



  
% \appendix     % the following sections will be numerated as appendices

% \begin{thebibliography}{10}
% \bibitem{ labelx } Author, eth  % for cite: \cite{ labelx }
% \end{thebibliography}

% text in two columns:
% \begin{tabular}{p{5cm} p{5cm}}
% paragraph1  &  paragraph2\\
% \end{tabular}


% EQUATIONS IN TWO COLUMNS:
%% \begin{align}
%% \begin{aligned}
%%   \minimize &x+y+z\\
%% \st&a_1\leq x\leq b_1\\
%% &a_2\leq y+z\leq b_2
%% \end{aligned}
%% \hspace{3cm}
%% \begin{aligned}
%%   \minimize &x+y+z\\
%% \st&a_1\leq x\leq b_1\\
%% &a_2\leq y+z\leq b_2
%% \end{aligned}
%% \end{align}

%% COLOR BOXES
%% \begin{colbox}{red}
%% TEXT, EQUATIONS, ETC
%% \end{colbox}

%% FUNCTIONS IN EMACS TO COMPILE

%% A) BIBTEX + PDFLATEX:
%%  (defun compileltx ( )
%% (interactive)
%% (progn
%%  (save-buffer) 
%%  (setq name (buffer-name))

%%   (progn 
%%     (setq posdot (string-match "\\." name ))
%%     (setq pdfname (concat (substring name 0  posdot) ".pdf" ) ) 

%%  (setq posdot (string-match "\\." name ))
%%  (setq auxname (concat (substring name 0  posdot) ".aux" ) )

%% (call-process "bibtex" nil "bibtex"  nil auxname) 

%% (setq outvalue (call-process "pdflatex" nil "pdflatex"  nil name) )
%% (if (> outvalue 0) (switch-to-buffer "pdflatex")
%%   (progn 
%%     (setq posdot (string-match "\\." name ))
%%     (setq pdfname (concat (substring name 0  posdot) ".pdf" ) )
%% ; (call-process "evincescript.sh" nil  nil nil pdfname) 
%%     (start-process "my-process" "foo" "evince" pdfname))
%% )
%% )
%% )
%% )


%% (global-set-key "\C-c\C-w" 'compileltx)

% unset case insensitive search
%% (setq case-fold-search nil)




